How Well Do Multimodal Models Reason on ECG Signals?

While multimodal large language models offer a promising solution to the "black box" nature of health AI by generating interpretable reasoning traces, verifying the validity of these traces remains a critical challenge. Existing evaluation methods are either unscalable, relying on manual clinician review, or superficial, utilizing proxy metrics (e.g. QA) that fail to capture the semantic correctness of clinical logic. In this work, we introduce a reproducible framework for evaluating reasoning in ECG signals. We propose decomposing reasoning into two distinct, components: (i) Perception, the accurate identification of patterns within the raw signal, and (ii) Deduction, the logical application of domain knowledge to those patterns. To evaluate Perception, we employ an agentic framework that generates code to empirically verify the temporal structures described in the reasoning trace. To evaluate Deduction, we measure the alignment of the model's logic against a structured database of established clinical criteria in a retrieval-based approach. This dual-verification method enables the scalable assessment of "true" reasoning capabilities.

==> utils/scratchwork.tex <==
    % \textbf{Assessment Results for \projectname Perception.} The strong overall results of \projectname across both Supporting and Assessment show that our data science agent is able to accurately identify signal that are and are not there.   
    % Supporting assessment measures the alignment with ground truth cardiologist ECG notes; Adversarial assessment permutes the ground truth by swapping antonyms (e.g. Wide $\leftrightarrow$ Narrow QRS). Standard deviation was computed from 3 runs of each agent variation. Low standard deviations show that results are stable. and we dont need to rerun perception agent every time, helping us save on computational resources. 
    
    
    % With our team of physicians, we manually evaluated the failed reasoning traces in the validation set to categorize error sources. 
    Out of a total count of XXX errors, 38\% stem from the segmentation tool, while 25\% are borderline cases. 
    Notably, in 17\% of cases the code is correct while the MIMIC note is wrong.
    The distribution suggests our perception mechanism is highly reliable and capable of auditing errors in human-annotations.
    \ef{add total count here}
    
    
    \caption{\textbf{Sample output of Claude (Plot).} With the lower perception but high deduction performance, this implies that Claude is not able to reason precisely. Instead first getting the correct answer, then producing reasoning post hoc. This is why technically, various conditions such as "deep QS complexes" are in fact indicative of myocardial infarction, but that cannot be used as a diagnostic criteria, because it simply is not present in the ECG. This has concerns in the trustworthiness of the approach, as the reasoning may in fact be an illusion, which has serious problems for the health domain. 



% \begin{itemize}[leftmargin=*,noitemsep, topsep=0pt]
%     \item {Exact Quote Extraction:} Identifying verbatim excerpts that define the diagnosis; and
%     \item {Structured Synthesis:} Summarizing and standardizing the criteria into a consistent format.
% \end{itemize}



\begin{table}[]
\centering
\captionof{table}{\textbf{Comparison of Various Evaluation Methods for Multimodal Reasoning.}
\harish {change title for multiple valid reasoning s}
} 
\vspace{-1mm}
\label{tab:assessment_comparison_compact}
\setlength{\tabcolsep}{1mm}
\resizebox{\linewidth}{!}{%
% CHANGE: Replaced 'l' with '>{\raggedright\arraybackslash}m{2.8cm}'
% This forces the first column to vertically center ("middle") its content
\begin{tabular}{l >{\centering\arraybackslash}m{2.6cm} >{\centering\arraybackslash}m{2.6cm} >{\centering\arraybackslash}m{2.6cm} >{\centering\arraybackslash}m{2.6cm} >{\centering\arraybackslash}m{2.6cm}} 
\toprule[1.5pt]
% Headers
Method & 
\makecell{\textbf{Applicable to} \\ \textbf{Health Data}} & 
\makecell{\textbf{Assesses} \\ \textbf{Reasoning Text}} & 
\makecell{\textbf{Inspects Non-} \\ \textbf{Text Modality}} & 
\makecell{\textbf{Allows Multiple} \\ \textbf{Valid Reasonings}} & 
\textbf{Reproducible} \\
\midrule

% Method 1
\makecell[l]{Step-wise Decomposition\\ \citep{zhou2025mpbench, jiang2025mmecot}} & 
& $\cmark$ & $\cmark$ & & $\cmark$ \\
\cmidrule(lr){1-6}

% Method 2
\makecell[l]{Question-Answering\\ \citep{oh2023ecgqa, yue2024mmmu}} & 
$\cmark$ & & & & $\cmark$ \\
\cmidrule(lr){1-6}

% Method 3
\makecell[l]{Zero-shot Classification\\ \citep{chow2024towards, zhang2025sensorlm}} & 
$\cmark$ & & & & $\cmark$ \\
\cmidrule(lr){1-6}

% Method 4
\makecell[l]{n-gram Match\\ \citep{li2024sensorllm}} & 
$\cmark$ & $\cmark$ & & & $\cmark$ \\
\cmidrule(lr){1-6}

% Method 5
\makecell[l]{Expert Assessment\\ \citep{langer2025opentslm, dai2025qoqmed}} & 
$\cmark$ & $\cmark$ & $\cmark$ & $\cmark$ & \\
\cmidrule(lr){1-6}

% Ours
\makecell[l]{\vspace{-5pt} \projectname \ (Ours)}  & 
$\cmark$ \vphantom{\makecell{A \\ B}} & $\cmark$ \vphantom{\makecell{A \\ B}} & $\cmark$ \vphantom{\makecell{A \\ B}} & $\cmark$ \vphantom{\makecell{A \\ B}} & $\cmark$ \vphantom{\makecell{A \\ B}} \\

\bottomrule[1.5pt]
\end{tabular}%
}
\vspace{3pt}
\vspace{-2mm}
\end{table}



\textbf{Metrics.} 
% We evaluate the alignment between the model's reasoning and the retrieved expert criteria using standard information retrieval metrics. 
We employ standard thretrieval metrics such as: \textit{(i)} top-$k$ accuracy, which measures whether the correct diagnostic label appears \textit{at least once} among the top-$k$ retrieved articles. 
This indicates if the reasoning is sufficiently distinct to surface the correct pathology. 
 \textit{(ii)} Precision@$k$ measures the proportion of the top-$k$ retrieved articles that match the correct ground-truth label. 
This effectively grades the {specificity} of the reasoning. 
A higher precision implies the model's logic is consistently mapping to the correct disease rather than ambiguous or unrelated conditions.



\begin{table*}[t]
\centering
\caption{\textbf{Validation of \projectname Deduction.} We evaluate the alignment of our retrieved medical references used during Deduction against diagnostic criteria independently authored by three physicians. The full \projectname pipeline consistently performs well with high Top-$k$ Accuracy and Precision@$k$. This confirms that our data extraction agent effectively captures the nuanced ``clinical logic" required by experts, serving as a robust proxy for clinical consensus.}
\label{tab:physician_validation}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccccccccccccc}
\toprule
\textbf{\makecell[l]{Deduction \\ Validation}} & 
\multicolumn{5}{c}{\makecell{\textbf{Physician A}}} & 
\multicolumn{5}{c}{\makecell{\textbf{Physician B}}} & 
\multicolumn{5}{c}{\makecell{\textbf{Physician C}}} \\
\cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
& {\contour{black}{$^{\uparrow}$}Top-1} & {\contour{black}{$^{\uparrow}$}Top-5} & {\contour{black}{$^{\uparrow}$}Top-10} & {\contour{black}{$^{\uparrow}$}Precis} & {\contour{black}{$^{\uparrow}$}Precis} 
& {\contour{black}{$^{\uparrow}$}Top-1} & {\contour{black}{$^{\uparrow}$}Top-5} & {\contour{black}{$^{\uparrow}$}Top-10} & {\contour{black}{$^{\uparrow}$}Precis} & {\contour{black}{$^{\uparrow}$}Precis} 
& {\contour{black}{$^{\uparrow}$}Top-1} & {\contour{black}{$^{\uparrow}$}Top-5} & {\contour{black}{$^{\uparrow}$}Top-10} & {\contour{black}{$^{\uparrow}$}Precis} & {\contour{black}{$^{\uparrow}$}Precis} \\
& {Acc} & {Acc} & {Acc} & {@5} & {@10}
& {Acc} & {Acc} & {Acc} & {@5} & {@10}
& {Acc} & {Acc} & {Acc} & {@5} & {@10} \\
\cmidrule(lr){1-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}

\textbf{\projectname}    & 0.830 & 0.982 & 1.000 & 0.763 & 0.687 & 0.789 & 0.989 & 1.000 & 0.780 & 0.706 & 0.790 & 0.958 & 1.000 & 0.746 & 0.702 \\
\midrule
\multicolumn{5}{l}{\textit{Ablations}} \\
w/o Quote Extract  & 0.725 & 0.959 & 0.977 & 0.658 & 0.629 & 0.825 & 0.989 & 1.000 & 0.695 & 0.651 & 0.724 & 0.946 & 0.988 & 0.699 & 0.636 \\
w/o Struct. Extract   & 0.765 & 0.929 & 0.970 & 0.652 & 0.594 & 0.743 & 0.989 & 0.989 & 0.734 & 0.652 & 0.771 & 1.000 & 1.000 & 0.728 & 0.660 \\
w/o two LLMs & 0.762 & 0.970 & 0.994 & 0.718 & 0.646 & 0.722 & 0.938 & 1.000 & 0.700 & 0.656 & 0.744 & 0.955 & 0.994 & 0.688 & 0.645 \\
w/o Extraction Agent    & 0.395 & 0.829 & 0.928 & 0.422 & 0.346 & 0.373 & 0.897 & 0.989 & 0.397 & 0.353 & 0.470 & 0.899 & 0.946 & 0.416 & 0.364 \\
\midrule
\multicolumn{5}{l}{\textit{Sources}} \\
w/o LITFL               & 0.769 & 0.959 & 0.970 & 0.696 & 0.644 & 0.801 & 0.966 & 0.989 & 0.675 & 0.646 & 0.704 & 0.909 & 1.000 & 0.675 & 0.645 \\
w/o ECGPedia            & 0.831 & 1.000 & 1.000 & 0.774 & 0.705 & 0.778 & 0.989 & 1.000 & 0.773 & 0.688 & 0.789 & 0.958 & 1.000 & 0.730 & 0.689 \\
w/o Wikipedia           & 0.764 & 0.917 & 1.000 & 0.680 & 0.632 & 0.706 & 1.000 & 1.000 & 0.755 & 0.683 & 0.736 & 0.917 & 1.000 & 0.705 & 0.683 \\
w/o WikiEM              & 0.776 & 0.929 & 0.970 & 0.695 & 0.650 & 0.757 & 0.989 & 1.000 & 0.795 & 0.704 & 0.765 & 0.958 & 1.000 & 0.728 & 0.687 \\
\bottomrule
\end{tabular}
}
\end{table*}



\emph{C) Data Extraction Agent}. We utilize a Data Extraction agent to parse through the scraped articles and preprocess the text to identify sets of diagnostic criteria that are sufficient for a given condition. Using an agent here is essential because otherwise there is too much noise and irrelelvant information in each article. Additionally, because we just scraping the top 5 search results, not all of the articles may be directly relevant to the diagnosis label. As such, we can see in the row "w/o Extraction Agent" in Table \ref{tab:physician_validation}, performance drops signficantly acrosss all physicians.

In this approach, we use multiple differnet approaches in parallel to extract differetnt massaged versions of the raw articles in paralle. To do so, we utilize two different agents in parallel. The first agent is designed to extract raw \emph{exact} quotes from the original articles and the second agent is designed to synthesize information together and standardize the criteria in a specific way. The exact prompts used for each agent can be found in the Appendix \ref{appendix:deduction}. These data extraction agent was powered utilizing with the current state-of-the-art LLMs, Claude 4.5 Opus \citep{anthropic2024claudeopus45} and GPT 5.2 Pro \citep{openai2025gpt52}, so that in total the data extraction agents extracted data 4 times, 2 for each method and 2 for each agent.  

In our ablation table, we can see that combining all of these extractions together leads to the best performance because it helps capture a better heterogenous corpus of text to be compared to in this large database. Therefore, there is not one set best approach, where using only structured extraction or using only quote extraction is best or using a particular LLM model is best. Pushing them all together is best. 


\begin{figure*}[t!] % The '*' tells LaTeX to span both columns
    \centering
    \begin{tcolorbox}[
        % colback=white,
        % colframe=gray!80!black,
        title=\textbf{Abbreviated Perception Verification Prompt},
        % fonttitle=\bfseries\sffamily,
        boxrule=0.8pt,
        arc=2mm,
        left=6pt, right=6pt, top=6pt, bottom=6pt % Increased padding slightly for wide view
    ]
    % \small\sffamily
    You are an ECG analysis expert, Cardiac Electrophysiologist, and a Data Scientist.
    
    \textbf{Input Data}
    \begin{itemize}[leftmargin=*, noitemsep, topsep=0pt]
        \item \texttt{ecg\_signal} (np.array): Shape (12, 5000), 12-lead 10s ECG, fs=500Hz.
        \item \texttt{ecg\_features\_dict} (Dict): Pre-computed features keyed by lead (e.g., 'I', 'V1'). Contains scalars (e.g., \texttt{avg\_QT\_interval}) and arrays (e.g., \texttt{RR\_intervals}).
    \end{itemize}
    
    \textbf{Target Reasoning Trace:} \texttt{\{reasoning\_trace\}}
    
    \textbf{Task Definition}
    \begin{enumerate}[leftmargin=*, noitemsep, topsep=0pt]
        \item Extract Findings (JSON): Parse the trace for verifiable signal properties (rhythm/morphology). Ignore high-level diagnoses. Output a JSON dict where \texttt{key}=finding name and \texttt{value}=list of exact quotes from the trace.
        \item Write Verification Code (Python): Write \texttt{verify\_perception(ecg\_signal, ecg\_features\_dict)}. Return a boolean dictionary checking if the specific claims in the quotes are supported. \looseness -1
    \end{enumerate}
    
    \textbf{Output Schema (One JSON block + One Python block)}

    \begin{minipage}{0.48\textwidth} % Split example into side-by-side columns
        \textit{JSON Example:} \vspace{-7pt}
        \begin{minted}[fontsize=\scriptsize, baselinestretch=0.9]{json}
{
  "Sinus Tachy": ["Heart rate >100 bpm"], 
}
        \end{minted}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \textit{Python Example:}  \vspace{-7pt}
        \begin{minted}[fontsize=\scriptsize, baselinestretch=0.9]{python}
def verify_perception(ecg_signal, ecg_features_dict):
    findings_checks = {}
    hr = ecg_features_dict['II']['avg_heart_rate']
    findings_checks['Sinus Tachy'] = bool(hr > 100)
    return findings_checks
        \end{minted}
    \end{minipage}
    
    \end{tcolorbox}
    \caption{\textbf{Abbreviated Prompt for Data Science Agent During Perception Verification.}}
    \label{fig:system_prompt}
\end{figure*}



In order to scrape articles from each of these resources, we utilize the Google Search API. Given each set of labels in the PTB-XL dataset, 

(e.g. "atrial fibrillation site:https://litfl.com/")




because PTB-XL is great. PTB-XL is a state-of-the-art benchmarking dataset, that proposes a taxonomy of labels that we utilize based on form, diagnosis, rhythm, that we will utilize in our downstream evaluations of various multimodal language models. Their labels are comprehensive covering a wide range of conditions, and thus serve as a strong basis of differnet labels we should try to get diagnostic criteria from.  


The PTB-XL labels in fact form a superset of both of our downstream datasets, ECG-QA and MIMIC-IV




We operationalize this idea with a Retrieval-Augmented Generation (RAG) approach. First, we construct a comprehensive database of clinical literature, and then retrieve the top-$k$ reference articles most semantically similar to the reasoning trace to be evaluated.




Then, we compute a composite similarity score from the retrieved articles, strictly penalizing any matches to incorrect diagnoses by zeroing out their contribution. This yields a robust deduction score that reflects the reasoning trace's validity against the broader body of clinical consensus. Unlike traditional metrics such as BLEU, which rely on rigid n-gram overlap, this embedding-based approach captures nuanced semantic relationships, allowing for valid comparisons even when different terminology is used to describe the same underlying logic. Furthermore, while standard evaluation typically compare against a single reference trace, our framework compares the output against a large clinical database. This distinction is critical given the documented variability in physicians' ECG interpretation \citep{mccabe2013physician, cook2020accuracy, magee2014reliability}. 

We construct our reference database from a diverse corpus of authoritative cardiology resources, capitalizing on the fact that medical diagnoses are finite and historically been exhaustively documented. Our specific resources are below: 
% This includes three primary sources: medical textbooks, resident training materials, and case reports. Textbooks provide the formal criteria used for differential diagnosis; training materials offer clear, canonical examples; and case reports capture the nuance of rare or complex presentations. This multi-source approach ensures that the evaluator can verify reasoning traces ranging from standard textbook logic to the subtle deductions required for atypical cases.



\vspace{-3mm}
\begin{itemize}[leftmargin=*,noitemsep]
\item \href{https://litfl.com/ecg-library/diagnosis/}{\textbf{LITFL ECG Clinical Library:}} Serves as the "gold standard" for visual recognition in acute care. We use it to establish the canonical visual criteria (e.g., "De Winter’s T-waves"), providing a baseline for what a pathology \textit{should} look like.
\item \href{[https://pubmed.ncbi.nlm.nih.gov/?term=%28cardiology%29+AND+%28%28ecg%29+OR+%28ekg%29%29+AND+%28case+report%29&sort=](https://pubmed.ncbi.nlm.nih.gov/?term=%28cardiology%29+AND+%28%28ecg%29+OR+%28ekg%29%29+AND+%28case+report%29&sort=)}{\textbf{PubMed Case Reports:}} We aggregate historical and highly-cited case reports to capture "first principles" derivation of diagnoses. This ensures the evaluator can verify reasoning for atypical presentations often skipped by standard textbooks.
\item \href{[https://en.wikipedia.org/wiki/Electrocardiography](https://en.wikipedia.org/wiki/Electrocardiography)}{\textbf{Wikipedia:}} Represents the broadest tier of medical consensus. We include high-quality cardiology articles to capture general definitions and widely accepted standard-of-care descriptions that serve as a baseline for common knowledge.
\item \href{[https://en.ecgpedia.org/](https://en.ecgpedia.org/)}{\textbf{ECGpedia:}} A specialized, community-driven knowledge base dedicated solely to electrocardiography. Similar to LITFL but with a broader community focus, it provides diverse examples of morphological variations for common rhythms.
\item \href{[https://wikiem.org/wiki/Category:ECG](https://wikiem.org/wiki/Category:ECG)}{\textbf{WikiEM:}} Focused on Emergency Medicine, this resource prioritizes rapid triage and decision-making protocols. We use it to validate reasoning traces that involve urgent clinical actions or "red flag" identification logic.
\end{itemize}



This dataset contains approximately 600,000 diagnostic 12-lead ECG recordings (10 seconds duration, sampled at 500 Hz) collected from nearly 160,000 unique patients directly paired to expert cardiologist reports. 



However, classical rule-based algorithms \citep{emrich2024physiology, alarcon2025optimization} often fail on pathological data despite high benchmark scores on healthy signals \citep{joung2024deep}. As shown in Table \ref{tab:validation_results}, these methods degrade performance by frequently hallucinating features—most notably detecting phantom P-waves in Atrial Fibrillation. To ensure robustness across pathologies, we instead utilize a state-of-the-art deep learning segmentation model \citep{park2025semisegecg} explicitly trained on diverse clinical cohorts."



% \begin{table}[t]
% \centering
% \caption{\textbf{Semantic Mappings for Adversarial Validation.} We invert specific clinical findings using these mutually exclusive semantic sets to test for false positives in our Perception Evaluation.}
% \label{tab:adv_map}
% \small
% \begin{tabular}{p{0.6\linewidth} p{0.35\linewidth}}
% \toprule
% \textbf{Antonyms} & \textbf{Notes} \\
% \midrule
% Wide $\leftrightarrow$ Narrow & e.g. Wide QRS  \\ \addlinespace
% Elevation $\leftrightarrow$ Depression & e.g. ST Elevation \\ \addlinespace
% Regular $\leftrightarrow$ Irregular & e.g. Regular rhythm \\ \addlinespace
% Upright $\leftrightarrow$ Inverted & e.g. Inverted P wave \\ \addlinespace
% Prolonged $\leftrightarrow$ Shortened & e.g. Prolonged PR \\ \addlinespace
% Left $\leftrightarrow$ Right & e.g. Left axis deviation \\ \addlinespace
% High $\leftrightarrow$ Low & e.g. High QRS voltage \\ \addlinespace
% Poor $\leftrightarrow$ Normal & e.g. Poor progression \\ \addlinespace
% \{Absent, Flat\} $\leftrightarrow$ \{Present, Peak\} & e.g. P waves absent \\ \addlinespace
% % Anterior $\leftrightarrow$ Inferior $\leftrightarrow$ Lateral $\leftrightarrow$ Posterior & e.g. Anterior MI \\ \addlinespace
% \{Fusion, Fused\} $\leftrightarrow$ \{Distinct, Capture\} & e.g. Fused T waves \\ \addlinespace
% Sinus Rhythm $\leftrightarrow$ Sinus Bradycardia $\leftrightarrow$ Sinus Tachycardia $\leftrightarrow$ Atrial Fibrillation $\leftrightarrow$ Atrial Flutter $\leftrightarrow$ Junctional Rhythm & Different heart rate speeds and rhythms. \\
% \bottomrule
% \end{tabular}
% \end{table}



% \begin{table}[t]
% \centering
% \caption{\textbf{Validation results for ECG perception.} Supporting metrics measure the alignment with ground truth, while Adversarial metrics measure the rate of critical hallucination/disagreement.}
% \label{tab:validation_results}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lcccc}
% \toprule
% \textbf{\makecell[l]{Perception \\ Validation}} & 
% \multicolumn{3}{c}{\textbf{\makecell{\contour{black}{$^{\uparrow}$}Supporting Validation}}} & 
% \textbf{\makecell{\contour{black}{$^{\downarrow}$}Adversarial \\ Validation}} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-5}
% & \textbf{$\text{Acc}_{\text{Micro}}$} & \textbf{$\text{Acc}_{\text{Macro}}\text{@50}$} & \textbf{$\text{Acc}_{\text{Macro}}\text{@100}$} & \textbf{$\text{Acc}_{\text{Macro}}\text{@100}$} \\
% & \scriptsize\makecell{Total \% \\[-0.3ex] Verified} & \scriptsize\makecell{\% of Traces with \\[-0.3ex] 50\% Verified} & \scriptsize\makecell{\% of Traces with \\[-0.3ex] 100\% Verified} & \scriptsize\makecell{\% of Traces with \\[-0.3ex] 100\% Verified} \\
% \midrule

% \textbf{\projectname}              & $0.830{\scriptscriptstyle \pm .000}$ & $0.939{\scriptscriptstyle \pm .002}$ & $0.669{\scriptscriptstyle \pm .009}$ & $0.124{\scriptscriptstyle \pm .005}$ \\
% \midrule

% w/ Single-step                 & $0.631{\scriptscriptstyle \pm .014}$ & --                                   & $0.631{\scriptscriptstyle \pm .014}$ & $0.138{\scriptscriptstyle \pm .003}$ \\
% w/ Multi-Agent                 & $0.715{\scriptscriptstyle \pm .006}$ & $0.842{\scriptscriptstyle \pm .005}$ & $0.463{\scriptscriptstyle \pm .017}$ & $0.088{\scriptscriptstyle \pm .008}$ \\
% w/ Rule Segment                & $0.754{\scriptscriptstyle \pm .010}$ & $0.913{\scriptscriptstyle \pm .006}$ & $0.581{\scriptscriptstyle \pm .003}$ & $0.128{\scriptscriptstyle \pm .005}$ \\
% w/o Helper Tools               & $0.688{\scriptscriptstyle \pm .020}$ & $0.816{\scriptscriptstyle \pm .017}$ & $0.463{\scriptscriptstyle \pm .019}$ & $0.141{\scriptscriptstyle \pm .003}$ \\
% \bottomrule
% \end{tabular}
% }
% \end{table}
% % & \textbf{MicroAcc} & \textbf{MacroAcc@50} & \textbf{MacroAcc@100} & \textbf{MacroAcc@100} \\



\emph{C) Finally, we choose our backend LLM}. While smaller LLMs seem do well, their performance is due to hallucinations. See Figure, which shows an example verify\_perception function for both Gemini 3 pro and flash. Gemini 3 actually tries to write code, whereas Flash, handwaves this away. This can clearly be seen in the "Adversarial Validation" results, where the accuracy remains quite high, showing a high false positive rate. Inspection of results show that weaker models, fail because they are unable to write sufficient functions that test for domain knowledge. 

Further prompt engineering did not help prevent this from occuring. 






In addition to this tool, we provide other functions, such as "calculate\_RR\_interval()", `calculate\_st\_interval` to calculate common features used inn the annalysis. These functions are crucial and are what physicians use when interpretting the signnal. Additionally, one crucial, yet obvious in hindsight fucntion, we included was `lead\_to\_index` function, which returns the leads per signal. This is crucial because this each lead measures a different dimennsion of the heart, it is obvious in hindsight with domain knowledge, but somethingn that can be easily overlooked without domain knowledge, especially because in MIMIC-IV-ECG the AVL lead is put before the AVR lead, but this is reversed in PTB-XL's ECG data. there is a set order, but mimic-iv uses a differnet order





\emph{A) First, we craft specific tools for our data sciennce agent to be able to use.} The purpose here is to lower the abstraction barrier. This is because our goal is for our data science agent to be as correct as possible, we assume that when the data sciennce agennt writes verification code, the code is correct so that we can use it as a evaluation mechanism. 

The clinical lexicon of ECG reports focus on segmennting out differnet portions of the ECG signal that capture specific features.  For example, "asdf", "asdf", and "asdf. Each of these notes rely on the assumptionn. 

There have been a few advances in this field, focusing on using ECG segmentation algorithsm. It is very tricky to do so because most ECG segmentation (or called delineation from the classical field) algorithms have been classically trained on "clean" and "healthy" data, where it is easy to identify specific P waves. In our results, we demonsntrate that using these classical, naive, rules-based segmentation algorithms perform quite poorly annd make false claims due the underlying tools being wrong. For example, one condition of atrial fibrillation is that P-waves are not present, but these classical algorithms assume a clean signal and identify phantom P-waves. Instead, we utilize a recent, state-of-the-art deep learning approach as a tool, specifically trained for segmenntation of healthy and unhealty individuals. 


The clinical lexicon of ECG interpretation relies heavily on segmenting distinct portions of the signal. For example, common findings in cardiologist notes are "prolonged PR interval", "wide QRS complex". and "ST segment elevation" all depend on the accurate delineation of the P, Q, R, S, and T ECG wave boundaries. However, reliable segmentation is non-trivial. Classic rules-based ECG segmentation algorithms have low computational overhead but use physiological assumptions \citep{emrich2024physiology, jaeger2024systematic} or transforms to decompose the signal into specific wavelets \citep{alarcon2025optimization}. This results in strong performance on standard benchmarks that are composed of primarily healthy ECGs, but much worse on pathological ECGs that exhibit unexpected behaviors \citep{joung2024deep}. This can be seen in the "w/ Rule-based Segmentation" line in Table \ref{tab:validation_results}, in which performance drastically decreases. One of the diagnostic criteria of Atrial fibrillation is the lack of P waves, but while inspecting our evaluation pipeline, we found that rules-based segmentation algorithms will very commonly hallucinate phantom P waves, causing the evaluation pipeline to incorrectly determine a "positive perception" result. Therefore, our approach utilizes an open state-of-the-artdeep learning segmentation model \citep{park2025semisegecg} explicitly trained on both healthy and pathological cohorts to ensure robust segmentation, which has been shown to be crucial for maintain strong segmentation performance on pathological ECGs \citep{joung2024deep}. 



The healthcare domain is particularly interesting because this is where reasoning capability is the most critical, yet it remains significantly underexplored. The ability to reason over health data is fundamental to building trustworthy systems for real-world clinical deployment \citep{lin2024machine}, but standard reasoning evaluation metrics (i.e. zero-shot prediction \citep{chow2024towards, zhang2025sensorlm}, QA accuracy \citep{oh2023ecgqa, yue2024mmmu}, BLEU score \citep{li2024sensorllm}, etc.) serve only as weak proxies for "true" reasoning. The most promising alternative, successfully applied in mathematics-based tasks, involves step-wise decomposition, where reasoning traces are broken down and quantitatively verified at each step \citep{zhou2025mpbench, jiang2025mmecot}. Unfortunately, this method translates poorly to healthcare. Unlike the rigid logic of mathematics, clinical interpretation is often ambiguous and cannot have the precisely annotated intermediate steps required for such granular evaluation. Their simplicity in evaluation targets may explain why prior research has shown these multimodal language models often suffer from accuracy collapse on complex tasks \citep{shojaee2025the}. 


Aligning modalities into the language domain allows for multimodal models to leverage the semantic capabilities derived from centuries of human development, for free. For instance, \emph{semantic similarity} enables \emph{zero-shot prediction} of unseen classes (i.e. predicting "snowboarding" from wearable signals when pre-trained with "skiing" captions \citep{zhang2025sensorlm}), and \emph{instruction following} enables some \emph{control} of the other modality (i.e. generating synthetic images from text descriptions \citep{ramesh2021dalle}). However, the ultimate goal of multimodal language alignment is achieving reasoning capability, where a model learns to interpret and analyze the other modality to reach a conclusion with a human-interpretable, logical reasoning trace. With "true" reasoning, multimodal models can contextualize the other modality within our existing semantic knowledge, enabling richer representations grounded in semantic understanding, along with better control and interpretability. Consequentially, reasoning is the definitive benchmark for assessing the quality of language alignment.



such as Humanities Last Exam, ARC-AGI-2, CharXiv, but these benchmarks are not satisfactory and do not assess the reasoning trace. Humanities Last Exam is a comprehensive "2,500 expert-level questions across a broad range of subjects." and CharXiv , but is just question-answering that only assess final answer accuracy. ARC-AGI-2

Large LLMs only benchmark their "reasoning" on blah and blah, but not reasoning.


only reasoning on math. For math, 


For example, 

Other multimodal models that can generate text output
SensorLM benchmarks 

The most promising alternative, successfully applied in mathematics-based tasks, involves step-wise decomposition, where reasoning traces are broken down and quantitatively verified at each step \citep{zhou2025mpbench, jiang2025mmecot}. Unfortunately, this method translates poorly to healthcare. Unlike the rigid logic of mathematics, clinical interpretation is often ambiguous and cannot have the precisely annotated intermediate steps required for such granular evaluation. Their simplicity in evaluation targets may explain why prior research has shown these multimodal language models often suffer from accuracy collapse on complex tasks \citep{shojaee2025the}. 



However, prior reasoning evaluationns are insufficient and reasoning capabilities are unknown. Within health, even if the multimodal reasoning models are designed with reasoning capabilities, nnone of them have been designed to evaluate reasoning. The ground truth is typically clinicians, but the evaluation is usually done post-hoc, 

Outside of health, multimodal models still only rarely evaluate reasoning. 

Unimodal 

Reasoning on modalities is very important because allows for interpretable innsights. This is especially useful for 



Aligning mod
Integrating language into multimodal models unlocks powerful capabilities, 


such as semantic similarity for zero-shot generalization (e.g., predicting "snowboarding" from signals after training on "skiing" \citep{zhang2025sensorlm}) and instruction following for controllable generation \citep{ramesh2021dalle}. However, the transformative potential of these models is most fully realized through reasoning—the ability to actively interpret and analyze non-linguistic data to reach a conclusion. Unlike simple mapping or alignment, reasoning enables models to produce human-interpretable, logical traces that contextualize raw signals within broader semantic knowledge. This capacity for structured analysis not only improves interpretability but also allows for richer, grounded representations, making reasoning a critical benchmark for the utility and reliability of multimodal systems.




The healthcare domain is particularly interesting because this is where reasoning capability is the most critical, yet it remains significantly underexplored. The ability to reason over health data is fundamental to building trustworthy systems for real-world clinical deployment \citep{lin2024machine}, but standard reasoning evaluation metrics (i.e. zero-shot prediction \citep{chow2024towards, zhang2025sensorlm}, QA accuracy \citep{oh2023ecgqa, yue2024mmmu}, BLEU score \citep{li2024sensorllm}, etc.) serve only as weak proxies for "true" reasoning. The most promising alternative, successfully applied in mathematics-based tasks, involves step-wise decomposition, where reasoning traces are broken down and quantitatively verified at each step \citep{zhou2025mpbench, jiang2025mmecot}. Unfortunately, this method translates poorly to healthcare. Unlike the rigid logic of mathematics, clinical interpretation is often ambiguous and cannot have the precisely annotated intermediate steps required for such granular evaluation. Their simplicity in evaluation targets may explain why prior research has shown these multimodal language models often suffer from accuracy collapse on complex tasks \citep{shojaee2025the}. 



"Although prior multimodal health models with reasoning capabilities have been developed \citep{dai2025qoqmed, langer2025opentslm}, their current evaluation frameworks remain insufficient for the health domain. While models like OpenTSLM and QoQ-Med validated a small subset of reasoning traces via trained clinicians, this manual approach is neither reproducible nor scalable. Consequently, new models cannot be validated against the same standard, effectively restricting progress to institutions with access to clinical experts and preventing fair cross-model comparisons. To address this gap, researchers often rely on objective proxies such as final classification accuracy, zero-shot performance, or BLEU scores. However, these metrics fail to constitute a unified benchmark for reasoning: they either measure only the final outcome—ignoring the validity of the derivation—or rely on superficial textual overlaps that do not capture the semantic correctness of clinical logic."



The healthcare domain is particularly interesting because this is where reasoning capability is the most critical, yet it remains significantly underexplored. The ability to reason over health data is fundamental to building trustworthy systems for real-world clinical deployment \citep{lin2024machine}, but standard reasoning evaluation metrics (i.e. zero-shot prediction \citep{chow2024towards, zhang2025sensorlm}, QA accuracy \citep{oh2023ecgqa, yue2024mmmu}, BLEU score \citep{li2024sensorllm}, etc.) serve only as weak proxies for "true" reasoning. The most promising alternative, successfully applied in mathematics-based tasks, involves step-wise decomposition, where reasoning traces are broken down and quantitatively verified at each step \citep{zhou2025mpbench, jiang2025mmecot}. Unfortunately, this method translates poorly to healthcare. Unlike the rigid logic of mathematics, clinical interpretation is often ambiguous and cannot have the precisely annotated intermediate steps required for such granular evaluation. Their simplicity in evaluation targets may explain why prior research has shown these multimodal language models often suffer from accuracy collapse on complex tasks \citep{shojaee2025the}. 


Aligning modalities into the language domain allows for multimodal models to leverage the semantic capabilities derived from centuries of human development, for free. For instance, \emph{semantic similarity} enables \emph{zero-shot prediction} of unseen classes (i.e. predicting "snowboarding" from wearable signals when pre-trained with "skiing" captions \citep{zhang2025sensorlm}), and \emph{instruction following} enables some \emph{control} of the other modality (i.e. generating synthetic images from text descriptions \citep{ramesh2021dalle}). However, the ultimate goal of multimodal language alignment is achieving reasoning capability, where a model learns to interpret and analyze the other modality to reach a conclusion with a human-interpretable, logical reasoning trace. With "true" reasoning, multimodal models can contextualize the other modality within our existing semantic knowledge, enabling richer representations grounded in semantic understanding, along with better control and interpretability. Consequentially, reasoning is the definitive benchmark for assessing the quality of language alignment.



such as Humanities Last Exam, ARC-AGI-2, CharXiv, but these benchmarks are not satisfactory and do not assess the reasoning trace. Humanities Last Exam is a comprehensive "2,500 expert-level questions across a broad range of subjects." and CharXiv , but is just question-answering that only assess final answer accuracy. ARC-AGI-2

Large LLMs only benchmark their "reasoning" on blah and blah, but not reasoning.


only reasoning on math. For math, 


For example, 

Other multimodal models that can generate text output
SensorLM benchmarks 

The most promising alternative, successfully applied in mathematics-based tasks, involves step-wise decomposition, where reasoning traces are broken down and quantitatively verified at each step \citep{zhou2025mpbench, jiang2025mmecot}. Unfortunately, this method translates poorly to healthcare. Unlike the rigid logic of mathematics, clinical interpretation is often ambiguous and cannot have the precisely annotated intermediate steps required for such granular evaluation. Their simplicity in evaluation targets may explain why prior research has shown these multimodal language models often suffer from accuracy collapse on complex tasks \citep{shojaee2025the}. 



However, prior reasoning evaluationns are insufficient and reasoning capabilities are unknown. Within health, even if the multimodal reasoning models are designed with reasoning capabilities, nnone of them have been designed to evaluate reasoning. The ground truth is typically clinicians, but the evaluation is usually done post-hoc, 

Outside of health, multimodal models still only rarely evaluate reasoning. 

Unimodal 

Reasoning on modalities is very important because allows for interpretable innsights. This is especially useful for 



Aligning mod
Integrating language into multimodal models unlocks powerful capabilities, 


such as semantic similarity for zero-shot generalization (e.g., predicting "snowboarding" from signals after training on "skiing" \citep{zhang2025sensorlm}) and instruction following for controllable generation \citep{ramesh2021dalle}. However, the transformative potential of these models is most fully realized through reasoning—the ability to actively interpret and analyze non-linguistic data to reach a conclusion. Unlike simple mapping or alignment, reasoning enables models to produce human-interpretable, logical traces that contextualize raw signals within broader semantic knowledge. This capacity for structured analysis not only improves interpretability but also allows for richer, grounded representations, making reasoning a critical benchmark for the utility and reliability of multimodal systems.




The healthcare domain is particularly interesting because this is where reasoning capability is the most critical, yet it remains significantly underexplored. The ability to reason over health data is fundamental to building trustworthy systems for real-world clinical deployment \citep{lin2024machine}, but standard reasoning evaluation metrics (i.e. zero-shot prediction \citep{chow2024towards, zhang2025sensorlm}, QA accuracy \citep{oh2023ecgqa, yue2024mmmu}, BLEU score \citep{li2024sensorllm}, etc.) serve only as weak proxies for "true" reasoning. The most promising alternative, successfully applied in mathematics-based tasks, involves step-wise decomposition, where reasoning traces are broken down and quantitatively verified at each step \citep{zhou2025mpbench, jiang2025mmecot}. Unfortunately, this method translates poorly to healthcare. Unlike the rigid logic of mathematics, clinical interpretation is often ambiguous and cannot have the precisely annotated intermediate steps required for such granular evaluation. Their simplicity in evaluation targets may explain why prior research has shown these multimodal language models often suffer from accuracy collapse on complex tasks \citep{shojaee2025the}. 



"Although prior multimodal health models with reasoning capabilities have been developed \citep{dai2025qoqmed, langer2025opentslm}, 

their current evaluation frameworks remain insufficient for the health domain. While models like OpenTSLM and QoQ-Med validated a small subset of reasoning traces via trained clinicians, this manual approach is neither reproducible nor scalable. Consequently, new models cannot be validated against the same standard, effectively restricting progress to institutions with access to clinical experts and preventing fair cross-model comparisons. To address this gap, researchers often rely on objective proxies such as final classification accuracy, zero-shot performance, or BLEU scores. However, these metrics fail to constitute a unified benchmark for reasoning: they either measure only the final outcome—ignoring the validity of the derivation—or rely on superficial textual overlaps that do not capture the semantic correctness of clinical logic."


and n-gram match metrics \citep{li2024sensorllm}. However, these metrics do not evaluate reasoning capbility, focusing on 




In order to attempt to solive this, both models are able report metrics on objective final classification accuracy. However, these metrics do not compare actual reasoning, but historically many methods will attempt to use this as a proxy. Zero-shot classification, Question answering, and  BLEU metrics remainn common, but none of these satisfactorily form a unified metric that can be used to compare reasonningn capabiliitesm due to either ... ... ...



Instead, the vast majority of existing datasets are annotated solely for final prediction accuracy. While some health-focused multimodal language models have validated their reasoning through manual expert review \citep{dai2025qoqmed, langer2025opentslm}, this approach is labor-intensive and ultimately unscalable to act as a unified benchmark.


Unlike other fields, medical knowledge is codified in comprehensive diagnostic criteria and detailed case reports. Additionally, because health sensors and imaging methods were specifically designed for human interpretation, the path to verifiable reasoning should, in theory, be clear. However, realizing this potential is elusive due to the lack of sufficient benchmarks. Despite extensive medical documentation, this medical knowledge is largely siloed, existing as isolated text rather than being paired with corresponding sensor data. Consequently, there is a lack of multimodal health datasets that include precise reasoning traces paired with raw data. 


"Despite these challenges, the health domain remains uniquely positioned for reasoning evaluation due to its extensive history of formalizing decision-making. Medical knowledge is not merely descriptive; it is rigorously codified into diagnostic criteria, clinical guidelines, and structured case reports designed explicitly to guide human interpretation. Because health sensors and imaging modalities were engineered to align with these human-readable frameworks, the theoretical path to verifiable reasoning is clearer here than in domains with less structured logic. However, realizing this potential remains elusive. While medical knowledge is vast, it remains largely siloed in textual form, separated from the raw sensor data it describes. Consequently, the field lacks the multimodal datasets necessary to ground AI reasoning in the very clinical standards designed to verify it."

